AnnoLLM: Making Large Language Models to Be Better Crowdsourced Annotators

Many natural language processing (NLP) tasks rely on labeled data to train machine learning models with high performance. However, data annotation is time-consuming and expensive, especially when the task involves a large amount of data or requires specialized domains. Recently, GPT-3.5 series models have demonstrated remarkable few-shot and zero-shot ability across various NLP tasks. In this paper, we first claim that large language models (LLMs), such as GPT-3.5, can serve as an excellent crowdsourced annotator when provided with sufficient guidance and demonstrated examples. Accordingly, we propose AnnoLLM, an annotation system powered by LLMs, which adopts a two-step approach, explain-then-annotate. Concretely, we first prompt LLMs to provide explanations for why the specific ground truth answer/label was assigned for a given example. Then, we construct the few-shot chain-of-thought prompt with the self-generated explanation and employ it to annotate the unlabeled data with LLMs. Our experiment results on three tasks, including user input and keyword relevance assessment, BoolQ, and WiC, demonstrate that AnnoLLM surpasses or performs on par with crowdsourced annotators. Furthermore, we build the first conversation-based information retrieval dataset employing AnnoLLM. This dataset is designed to facilitate the development of retrieval models capable of retrieving pertinent documents for conversational text. Human evaluation has validated the dataset's high quality.

==> sections/limitations.tex <==
\section{Limitations}
In this paper, we present the remarkable potential of AnnoLLM powered by GPT-3.5 to supplant crowdsourced annotators. Nevertheless, it is essential to acknowledge that our assessment of the proposed method's effectiveness is constrained by limited computational resources, restricting our investigation solely to GPT-3.5 series models.
To gain further insights, future endeavors should encompass supplementary experiments involving diverse language models, including PaLM and LLaMA. These additional investigations will undoubtedly enrich the understanding of the subject and expand the horizons of our research.


% There are two possible limitations of this work. 
% Firstly, limited by sufficient computational resources, we only verify the effectiveness of our proposed method on GPT series models. 
% Further experiments with other language models, such as PaLM and LLaMA are left as future work. 
% The second limitation is that the retrieved evidence may not be relevant to the input claim, which cannot provide useful information for correcting the factual errors within the input claim. 
% Since our work mainly focuses on improving factual error correction through the introduction of the pivot task, we leave the improvement of evidence retrieval to future work. 

